Towards a glaucoma risk index based on simulated hemodynamics from fundus images

Glaucoma is the leading cause of irreversible but preventable blindness in the world. Its major treatable risk factor is the intra-ocular pressure, although other biomarkers are being explored to improve the understanding of the pathophysiology of the disease. It has been recently observed that glaucoma induces changes in the ocular hemodynamics. However, its effects on the functional behavior of the retinal arterioles have not been studied yet. In this paper we propose a first approach for characterizing those changes using computational hemodynamics. The retinal blood flow is simulated using a 0D model for a steady, incompressible non Newtonian fluid in rigid domains. The simulation is performed on patient-specific arterial trees extracted from fundus images. We also propose a novel feature representation technique to comprise the outcomes of the simulation stage into a fixed length feature vector that can be used for classification studies. Our experiments on a new database of fundus images show that our approach is able to capture representative changes in the hemodynamics of glaucomatous patients. Code and data are publicly available in https://ignaciorlando.github.io.

==> arterial-encoding.tex <==

\subsection{Arterial tree extraction and processing}
\label{subsec:arterial-tree-encoding}

As indicated in Section~\ref{sec:introduction}, the simulations of the retinal hemodynamic are performed on the arterial trees. Thus, it is necessary to separate arteries and veins from the output of the vessel segmentation algorithm. Although there are several methods in the literature proposing different alternatives to perform this task in an automatic manner~\cite{abramoff2010retinal}, their application is out of the scope of this study. Instead, the arterial tree $T$ of each fundus photograph was manually identified by experienced ophthalmologists. \textcolor{red}{Check the justification of the manual annotation.}

\textcolor{red}{Rewrite the paragraph justifying why we remove the segments in the optic disc.}
%As usually there are pieces from the segmentation that lie inside the optic disc area and are left unlabeled as they are significantly overlapped and are difficult to classify into arteries or veins. To prevent introducing errors in the simulation of the hemodynamic process, all these pieces are removed using a coarse ellipsoidal representation of the optic disc manually drawn on the fundus photograph.

The centerlines of the arterial trees were afterwards identified using the skeletonization method proposed in~\cite{rumpf2002continuous}, resulting in a binary mask $T$ with $n_t$ connected components. Each connected component $T_i \in T$ has an associated root pixel $r_i$, which corresponds to the one closest to the optic disc area. To identify these points, the ellipsoidal mask of the optic disc is eroded using a disk of radius 2 pixels, and the pixels in the intersection between $T$ and the eroded mask are taken as roots.

Subsequently, each tree $T_i$ is modeled as a graph structure $G_i = \langle r_i, \mathcal{V}_i, \mathcal{E}_i \rangle $, where each node $v_j \in \mathcal{V}_i$ is a set of branching pixels in $T_i$, and each edge $e_k \in \mathcal{E}_i$ is a segment of centerlines pixels connecting two branching points. The pixels are automatically classified as part of a node or an edge in $G_i$ by analyzing the number of neighbors they have; thus, pixels with 3 neighbors are labeled as part of a node, and pixels with only 2 are mapped into segments. Notice that nodes might have more than a single associated pixels in some special scenarios.

As it will be further discussed in Section~\ref{subsec:arterial-model}, the hemodynamic simulation requires not only to count with the overall connectivity of the arterial trees but also with the approximate radius of each of the pixels in the structure. The vessel radius is approximated from the original segmentation by using the Euclidean transform, which is analogous to the 3D approach used in \cite{Antiga_CenterLine-2003}.

==> classification.tex <==

\subsection{Classification}
\label{subsec:classification}

==> cnn-based-features.tex <==

\subsection{Deep learning based features}
\label{subsec:deep-learning-based-features}

The key idea here is to validate if deep learning based features can be improved by the incorporation of functional knowledge obtained from our simulations of the retinal hemodynamics.

In order to do this, we took the VGG-M~\cite{chatfield2014return} architecture, pretrained with images from ImageNet~\cite{krizhevsky2012imagenet} as provided in the MatConvNet website, and we fine tune its weights using the images of the ORIGA-Light data set (Section~\ref{sec:materials}). We used 90\% of the images for fine tuning the weights of the CNN, and the remaining 10\% for validation. As the most evident changes are those manifested in the optic nerve head area, we crop the images around it to improve the discrimination ability of the CNN features. We used the manual annotations of the optic disc provided in the data set to control where to crop the images. The binary masks were dilated using a disk structuring element with a radius equivalent to 5\% the width of the image, in pixels. The input images are rescaled to 

==> hemodynamic-feature-encoding.tex <==

\subsection{Encoding of hemodynamic features}
\label{subsec:hemodynamic-feature-encoding}

==> materials.tex <==

\section{Materials}
\label{sec:materials}
\todo{{\carlos Nacho should move this section as is to the supplementary material, and then extract the most relevant info and put it as a second paragraph of section 2. Then, change the name of section 2 to Methods and Materials.}}
Our experiments were conducted on a new database of color fundus photographs, called LES-AV, that will be publicly released by the time of publication. It comprises 22 images of 22 subjects with ages ranging from 53 to 90 years (10 women). The images were captured using a Visucam ProNm fundus camera with a ZK-5 (PRO NM/ NMFA) 5 MP sensor, with resolutions of $30^\circ$ FOV and $1444 \times 1620$ pixels (21 images), and $45^\circ$ FOV and $1958 \times 2196$ pixels (one image), with each pixel $=$ 6 $\mu m$. The retinal vasculature was automatically segmented, first, and then manually refined and classified into arteries and veins by two ophthalmologists and a computer scientist. Ellipsoidal masks of the optic disc were also manually drawn for each image. 
% * <joao_breda@hotmail.com> 2018-02-28T11:16:59.861Z:
% 
% In our field, we usually place between brackets the initials of the authors that were tasked for this. But this a cultural thing in medical research. 
% 
% ^.




==> segmentation.tex <==

\subsection{Blood vessel segmentation}
\label{subsec:blood-vessel-segmentation}

We used a blood vessel segmentation method based on a patch-level trained U-Net architecture \cite{ronneberger2015u}, which has already shown promising results for this task in other applications~\cite{giancardo2017representation}. The model architecture is depicted in Figure~\ref{fig:unet}. We used max-pooling after each convolutional block, with kernels of size 2 pixels, followed by upsampling blocks composed of a convolutional block, a transposed convolution and a concatenation operation. Standard ReLUs are used as activation functions after each convolutional/deconvolutional layer. Batch normalization was introduced after all the convolutional layers to facilitate the convergence. Several regularization techniques were also applied to reduce overfitting, including dropout ($p = 0.5$) after the first convolution of each block, weight decay ($\lambda = 5 \times 10^{-4}$) and data augmentation.

\begin{figure}[t]
\label{fig:unet}
\includegraphics[width=\textwidth]{figures/u-net.pdf}
\caption{Schematic representation of our U-Net for blood vessel segmentation.}
\end{figure}

The U-Net was trained from scratch using randomly sampled patches of $64 \times 64$ pixels, extracted from preprocessed color fundus images. To enhance the contrast between the vasculature and the other areas of the retina, the contrast equalization method proposed in~\cite{van2016fast} was applied before extracting the patches. Moreover, the patches were collected in such a way that 50\% of them were centered on vascular areas and 50\% on background zones. 200.000 patches were used for each epoch, randomly shuffled in minibatches of size 32. We used the standard cross entropy loss as the objective function, optimized using SGD with momentum $\alpha = 0.99$, with an initial learning rate of 0.0001.







==> simulation.tex <==

\subsection{Simulation of the retinal hemodynamic}
\label{subsec:simulation}
